Shrinkwrap: Differentially-Private Query Processing in Private Data Federations

A private data federation is a set of autonomous databases that share a unified query interface offering in-situ evaluation of SQL queries over the union of the sensitive data of its members. Owing to privacy concerns, these systems do not have a trusted data collector that can see all their data and their member databases cannot learn about individual records of other engines. Federations currently achieve this goal by evaluating queries obliviously using secure multiparty computation. This hides the intermediate result cardinality of each query operator by exhaustively padding it. With cascades of such operators, this padding accumulates to a blow-up in the output size of each operator and a proportional loss in query performance. Hence, existing private data federations do not scale well to complex SQL queries over large datasets. We introduce Shrinkwrap, a private data federation that offers data owners a differentially private view of the data held by others to improve their performance over oblivious query processing. Shrinkwrap uses computational differential privacy to minimize the padding of intermediate query results, achieving up to 35X performance improvement over oblivious query processing. When the query needs differentially private output, Shrinkwrap provides a trade-off between result accuracy and query evaluation performance.

==> model.tex <==
\section{Privacy Model for Cardinalities}
\label{sec:model}

\eat{
We now discuss the privacy model used by \sysname for its privacy guarantees. First, we define our adversarial model and our usage of computational differential privacy. Second, we discuss how \sysname tracks privacy budget usage for each query, as well as multiple queries over time. Finally, we look at the cost of repeatedly applying differential privacy to intermediate results throughout an operator tree.

\subsection{Computational Differential Privacy}
\sysname offers an honest-but-curious threat model. Each data provider in the {\federation} honestly executes the provided \mpc protocol. Each provider however, is curious and will attempt to learn the sensitive data of other providers using side channels such as program counters and memory traces.

Current {\federation}s provide information-theoretic guarantees that guard against computationally unbounded adversaries. No matter how much time or computational power an adversary possesses, no information will be leaked. As part of our privacy-performance trade-off, we relax this guarantee to a computationally bounded scenario. \sysname guards against computationally bounded, polynomial time adversaries through the use of computational differential privacy (CDP). In previous work, CDP hides output cardinalities of individual relational operators, such as joins~\cite{He2017}. \sysname extends CDP to sequences of operators using Definition~\ref{def:cdp} and provides an optimized cost model.

\begin{definition}
IND-CDP privacy~\cite{Mironov:2009:CDP:1615970.1615981}

An ensemble $\{ f_{\kappa}\}_{\kappa\in \mathbb{N}}$ of randomized function
$f_{\kappa}: \mathcal{D} \rightarrow \mathcal{R}_{\kappa}$ provides $\epsilon_{\kappa}$-IND-CDP
if there exists a negligible function $negl(\cdot)$ such that for every nonuniform PPT TM $A$,
every polynomial $p(\cdot)$, every sufficiently large $\kappa \in \mathbb{N}$,
all data sets $D,D'\in \mathcal{D}$ of size at most $p(\kappa)$ such that $|(D-D')\cup(D'-D)|\leq 1$,
and every advice string $z_{\kappa}$ of size at most $p(\kappa)$, it holds that
\begin{displaymath}
\Pr[A_{\kappa}(f_{\kappa}(D)=1)]\leq e^{\epsilon_{\kappa}} \Pr[\Pr[A_{\kappa}(f_{\kappa}(D')=1)] + negl(\kappa)
\end{displaymath}
where $A_{\kappa}(x)$ for $A(1^{\kappa},z_{\kappa},x)$ and the probability is taken over the randomness of mechanisms $f_{\kappa}$ and adversary $A_{\kappa}$.
\label{def:cdp}
\end{definition}

Intuitively, Definition~\ref{def:cdp} states that a computationally bounded adversary cannot guess the true cardinality within a range of values specified by the privacy parameters $\epsilon$ and $\delta$. For \sysname, $\epsilon$ governs the amount of noise inserted into intermediate results, with higher values of $\epsilon$ indicating less noise and lower values indicating more noise. $\delta$ controls the offset of the noise. We use $\delta$ to increase the average noise inserted and ensuring that the noisy cardinality does not drop below the true cardinality with high probability.
}


Given a query tree, we would like to ensure the intermediate cardinalities of all operators in the tree are protected with computationally bounded differential privacy.
We define $q_i:\mathcal{D} \rightarrow \mathcal{R}$ as the output size of the sub-query rooted at operator $o_i$ in the query tree, i.e.  the intermediate cardinality query for operator $o_i$ in a given query tree.  We first show how to achieve this privacy guarantee using a variant of a classic differentially private mechanism for each intermediate cardinality with privacy cost of $(\epsilon_i,\delta_i)$. Then we will show in Section~\ref{sec:optimization} how to distribute privacy budgets among the operators in the query tree.

\subsection{Laplace Mechanism for Cardinalities}

For intermediate cardinalities, we draw the amount of noise to insert from a Laplace distribution according to Equation~\ref{def:noise}. To handle the case of negative noise, \sysname uses an additive offset, $\delta$.

\begin{definition}
Lap($\epsilon,\delta,\Delta q$))

For a given query $q:\mathcal{D}\rightarrow \mathcal{R}$,
a random variable follows the Lap($\epsilon,\delta,\Delta q$) distribution if it has a probability density function
\begin{displaymath}
\Pr[\eta=x] = p * e^{- (\epsilon/\Delta q)|x-\eta^0|}, \forall x \in \mathbb{Z},
\end{displaymath}
where
%\begin{displaymath}
$p = \frac{\epsilon/\Delta q - 1}{\epsilon/\Delta q+ 1}, \eta_0 = -\frac{\Delta q* ln((e^{\epsilon/\Delta q} + 1)(1-(1-\delta)^{1/\Delta q}))}{\epsilon}$
%\end{displaymath}
, and where $\Delta q$ is known as the sensitivity of the query, formally, defined as,
\begin{displaymath}
\Delta q = \max_{|D-D'|\cup |D'-D| = 1} |q(D)-q(D')|_1
\end{displaymath}
Intuitively, the sensitivity of a query is the maximum difference in the query output for any pairs of neighboring databases $D$ and $D'$.
\label{def:noise}
\end{definition}

\begin{theorem}
Given an intermediate cardinality query $q_i$ for operator $o_i$ in the query tree, adding $\max(\eta_i,0)$ number of dummy records,
where $\eta_i\sim$Lap($\epsilon_i,\delta_i, \Delta q_i$) satisfies $(\epsilon_i,\delta_i)$-IND-CDP.
\label{theorem:cdp}
\end{theorem}
\begin{proof}(sketch) The probability to draw a negative value from Lap($\epsilon_i,\delta_i, \Delta q_i$) is less than $1-(1-\delta_i)^{1/\Delta q_i}$.
For each neighboring pair, at most $\Delta q_i$ counts differ and fail to have the positive value, and hence the overall failing probability is $\delta_i$.
With $1-\delta_i$, the probability to have the same view from any neighboring databases is bounded by $e^{\epsilon_i}$.
\end{proof}

\sysname uses privacy parameters ($\epsilon, \delta$) provided by the client or a federation administrator. Their values will depend on the level of privacy guarantees required. CDP lets \sysname give tunable and provable privacy guarantees for {\federation} queries.


\subsection{Sensitivity Computation}
A intermediate result cardinality,  $q_i$, is the output size of the sub-query tree rooted at operator $o_i$. The sensitivity of $q_i$ depends on the operators in its sub-query tree, and we compute this as a function of  the stability of operators in the sub-query tree. The stability of an operator bounds the change in the output with respect to the change in the input of the operator. Formally,
\begin{definition}
Stability~\cite{mcsherry2009privacy}

A transformation operator is $c$-stable if for any two input data sets A and B,
\begin{displaymath}
|T(A) \ominus T(B)| \leq c \times |A \ominus B|
\end{displaymath}
\label{def:stability}
\vspace{-6mm}
\end{definition}

From Definition~\ref{def:stability}, we see that when the input of an operator changes, the stability of the operator bounds the change in the output. For non-join operators, the stability equals one. For join operators, the stability is equal to the maximum multiplicity of the input data. The sensitivity of the intermediate cardinality query $q_i$ can be recursively computed bottom up, starting from a single change in the input of the leaf node. More details can be seen in \cite{mcsherry2009privacy}.

For example, given a query tree shown in Figure~\ref{fig:sensitivity-tree}, the bottom two filter operators each have a stability of one, giving a sensitivity ($\Delta$q) of 1 at that point. Next, the first join has a stability of $m$ for the maximum input multiplicity, which increases the overall sensitivity to $m$. The following join operator also has a stability of $m$, which changes the sensitivity to $m^2$. Finally, the DISTINCT operator has a stability of 1, so the overall sensitivity remains $m^2$.

Using these principles, \sysname calculates the sensitivity for each operator in a query tree. We cover details of the implementation in Section~\ref{sec:design}.

\begin{figure} [t!]
\centering
\resizebox {!} {1.8in} {
\input{figures/sensitivity-tree}
}
\caption{Sensitivity analysis for running example}
\label{fig:sensitivity-tree}
%\vspace{-6mm}
\end{figure}




\eat{To this point, we have discussed privacy budget usage in terms of a single operator. However, queries typically involve composing multiple operators to form operator trees, which has a significant impact on the privacy used by a given query. Looking at Figure~\ref{fig:sensitivity-tree}, we can see the effect of operator composition on privacy parameters and query sensitivity.


In Figure~\ref{fig:sensitivity-tree}, we see that the magnitude of the privacy parameters increase upwards along the operator tree. Previous work has shown that sequential composition of operators results in an additive effect on the privacy parameters, while parallel composition, such as in joins, results in using the largest privacy parameters amongst the inputs~\cite{mcsherry2009privacy}. Privacy parameters increase along the tree to account for the cascading operators. Each time an operator evaluates an intermediate result, the client learns information about the source data. By repeatedly evaluating operators over that same input tables, clients gain more and more information about that data. \sysname accounts for the information leakage from multiple operators in a tree by increasing the privacy parameters accordingly.}




\cut{
\newtheorem{theorem}{Theorem}
\begin{theorem}
A mechanism that permits T adaptive interactions with a ${\delta}$-approximate, ${\epsilon}$-indistinguishable mechanism ensures ${\delta}T$-approximate ${\epsilon}T$-indistinguishability.
\label{theorem:composition}
\end{theorem}
\begin{proof}
Dwork et al.~\cite{Dwork2006} prove the additive nature of sequential composition for differential privacy. Below, we extend this proof to IND-CDP. \\
Assume that the result $x$ of mechanism $M$ is written as an ordered $T$-tuple, and lands in set $S$.
\begin{displaymath}
\Pr[x\in S] = \prod_{i \leq T} \Pr[x_i \in S_i \mid x_1,...,x_{i-1}]
\end{displaymath}
We can substitute the above into the definition of IND-CDP, where $x$ represents the result of $A_{\kappa}(f_{\kappa}(D))$ and $x_j$ represents $x_1,...,x_{i-1}$.
\begin{displaymath}
\prod_{i \leq T} \Pr[x_i \in S_i \mid x_j] \leq \prod_{i \leq T} (e^{\epsilon_{\kappa}} \Pr[x'_{i} \in S_i \mid x'_j] + negl(\kappa))
\end{displaymath}
Looking at $negl(\kappa)$, we see that it is only multiplied by itself, which gives a result that goes to zero, or a probability, which is at most one. This allows us to simplify the contribution of $negl(\kappa)$ to $Tnegl(\kappa)$, for the whole product. We can also now move $e^{\epsilon_{\kappa}}$ out of the product as $Te^{\epsilon_{\kappa}}$.
\begin{displaymath}
\prod_{i \leq T} \Pr[x_i \in S_i \mid x_j] \leq Te^{\epsilon_{\kappa}} \prod_{i \leq T} (\Pr[x'_{i} \in S_i \mid x'_j]) + Tnegl(\kappa)
\end{displaymath}
\end{proof}

Combining the stabilities of each operator in the tree yields the total sensitivity of the query. Previous works shows that for sequential composition of operators, stabilities are multiplied, while for parallel composition, the largest input stability is selected~\cite{mcsherry2009privacy}.

Armed with the knowledge of how operator composition affects both the privacy parameters, we can determine the amount of privacy budget consumed by any {\federation} query. Next, we see how \sysname optimizes privacy usage to improve query performance.
}

\subsection{Privacy Budget}
To support \sysname's non-information theoretic guarantees, we maintain a privacy budget for each relation in the federation.  When this privacy budget is depleted, the table will no longer be able to use \sysname. For example, say that a  medical researcher's {\federation} query joins a medication table with a diagnoses table to find incidences of heart disease that were treated with Aspirin. The true cardinality of the join's output would reveal the number of patients with heart disease to all data owners participating in the query's evaluation over \mpc. Using a differentially private cardinality would combat this leakage by only revealing a noisy version of the cardinality. However, if the researcher continued writing queries that included the join over the same tables and selection criteria, then over time the noisy cardinalities may be averaged together to obtain the true cardinality. Thus differential privacy can only be applied to a given data set a limited number of times. %We maintain a privacy budget for the data set.

\sysname tracks the privacy budget for each table separately. Whenever an operator uses a table, we deduct the privacy it used from the budget. In the example from Figure~\ref{fig:sensitivity-tree}, \sysname would deduct from the budgets of the medication and diagnosis tables. Our system maintains a single budget for each table, regardless of the query\textquotesingle s source. Other options, such as maintaining discrete budgets for different users have been explored in other systems~\cite{mcsherry2009privacy} and could be incorporated into \sysname.

The actual value of the privacy budget depends on the privacy parameters $\epsilon$ and $\delta$ shown in Definitions~\ref{def:eps-del-dp} and~\ref{def:cdp}. The privacy parameters bound the amount of privacy leaked by \sysname for each intermediate result, with $\epsilon$ controlling the magnitude of the noise and $\delta$ handling the additive offset. For a given intermediate result, \sysname sets $\epsilon$ to ensure that enough noise is added to the cardinality and $\delta$ to guarantee that the noisy cardinality never falls below the true cardinality with high probability.

\subsection{Composing Operators}
Similar to differential privacy, computationally differentially privacy also satisfies sequential compositions of operators.
\begin{theorem}[Sequential Composition]\label{theorem:seqcomp}
If $f_1$ and $f_2$ satisfy $(\epsilon_1,\delta_1)$-CDP and $(\epsilon_2,\delta_2)$-CDP,
then applying these two functions sequentially satisfies $(\epsilon_1+\epsilon_2,\delta_1+\delta_2)$-CDP.
\end{theorem}
\begin{proof}
Previous work by McSherry~\cite{mcsherry2009privacy} proves sequential composition of relational operators for CDP.
\end{proof}

In \sysname, all queries are sequential compositions, meaning we have to track the privacy usage of each operator. Every time an operator $o_i$ applies CDP, it must define the values of $\epsilon_i$ and $\delta_i$ used. These values each maintain their own budget, and every usage of ($\epsilon_i$,$\delta_i$)-CDP will subtract from their respective budgets. We describe the constraints on $\epsilon_i$ and $\delta_i$ for each operator $o_i$ in a query with privacy budget ($\epsilon$,$\delta$).
\begin{eqnarray}
\sum_{i=1}^{l} \epsilon_i \leq \epsilon & and & \sum_{i=1}^{l} \delta_i \leq \delta \nonumber
\end{eqnarray}
\eat{
\subsection{Protocol-agnostic Query Evaluation}
Researchers continue to make exciting advances in \mpc in the form of more efficient protocols and primitives.    \sysname will plan and execute queries such that it is agnostic to  the secure computation protocols with which it  evaluates  full-oblivious  operators.   Hence, we will be able to easily add new protocols to the query executor as they arise.  

\sysname's operators are expressed as secure circuits.  When selecting the protocol for a given query  operator, we need a generic way to  pick the best one for the job.  We will create a cost model and parameterize it for each of the secure protocols offered by \sysname.   We will estimate cost of an operator $op$ with $n_{gates}$ gates in its circuit, a maximum circuit depth of $d_{circuit}$, $n_{in}$ elements of input, and an output size of $n_{out}$ as:
$$cost_{op} = c_{in}*n_{in} + c_g*n_{gates} + c_d * d_{circuit} + c_{out} * n_{out}$$

This model is deliberately high-level and generic so that it will reflect the performance profile of most or all circuit-based \mpc protocols.  Hence, not all of its coefficients will be necessary for every protocol.  For example, some circuits may not use the circuit depth term. For binary operators, like joins and set intersections, we will add a second input size and coefficient for them.   When the query optimizer estimates the cost of a proposed query plan it will cycle through the protocols  available to it using this cost model to select an efficient one for it.

If a query plan uses multiple protocols and their data representations are different, the query planner  will automatically insert adapters between adjacent operators to  translate the secret-shared data like the ones in L1~\cite{schropfer2011l1}.  We will add this conversion overhead to our end-to-end cost estimate of a query plan. \cut{ Hence, when the optimizer is comparing one heterogeneous execution plan to other, equivalent ones (that will produce the same output) it will take this overhead into account.  We will go into more detail about this plan comparison step in the next section.}

  %Instead we focus on circuit-based operators because they accept arbitrary programs and compose easily with one another to support ad-hoc SQL statements.


%\todo{mention how there is a plethora of algorithms that do not use the circuit model, such as ones for PSI.  We do not consider these for now because they are usually not readily composable with other protocols and modeling their cost in the context of a SQL query where we have to consider many operator implementations and operator orderings.  Think more about what the concrete outcomes of that research would be.}


}

==> response.tex <==

\onecolumn
\begin{center}
    \textbf{\large{\sysname: Differentially-Private Query Processing in Private Data Federations}} \\
    \large{Revision Cover Letter} \\
    \textit{\normalsize{VLDB'19, Paper 114}} 
\end{center}

We would like to thank the reviewers for their helpful and constructive feedback on our submission. We greatly appreciate the opportunity to address the issues they raised.  As described below, this feedback significantly strengthened this paper. We now summarize our revisions to the paper. Note that we have renamed Distrustful Data Federation to Private Data Federation and honest broker to query coordinator in order to clarify their functions. In the revised paper, we highlight new or updated material in \change{blue}.


\ \\
{\bf \large{Meta Reviewer Comments}}
\begin{itemize}
    % 1. Provide more details on the trust model.
    \item MRD1: \textit{Trust Model Clarification}

    We added Section~\ref{sec:privacygoals} to clarify our trust model and summarize the model in Table~\ref{table:trustmodel}. Data owners require a privacy guarantee that the other parties (data owners, \hb and the client) are not able to reconstruct the private data they hold based on intermediate results of the query execution. In particular, we require data owners to have a differentially private view over the inputs of other data owners (formally defined in Def.~\ref{def:dp}). We support two output policies. Clients may be trusted (output policy 1) and allowed to see true answers to queries but must not learn any other information about the private inputs held by data owners. Clients may be untrusted (output policy 2), in which case they also are only permitted a differentially private view over the inputs. The \hb is an extension of the client and has the same privacy requirements.

    % 2. Address the reviewers' concern regarding the focus on 2 servers, as opposed to a more general solution (please see the summary comments for more details on the discussion).
    \item MRD2: \textit{$M$-Party Support}
    
    We added Section~\ref{sec:m-party} to discuss how our system generalizes to support execution across $M$ data owners. \sysname supports $M$ party computation by leveraging the associativity of our operators to convert all $M$ party computations into a series of binary computations. For example, assume we want to join to tables $R$ and $S$, which are horizontally partitioned across 3 data owners as $R1, R2, R3$, and $S1, S2, S3$. We can join across the 3 data owners as: $(R1 \bowtie S1) \cup (R1 \bowtie S2) \cup (R3 \bowtie S3) \cup (R2 \bowtie S1) \cup (R2 \bowtie S2) \cup (R2 \bowtie S3) \cup (R3 \bowtie S1) \cup (R3 \bowtie S2) \cup (R3 \bowtie S3)$. We can execute this series of binary joins using two party secure computation, then union the results. With this construction, we can scale \sysname out to any number of parties. However, this algorithm is not efficient due to naively carrying out $M^2$ secure computation operations for every $M$ parties we compute over. We leave performance improvements in this setting for future work.
    % 3. The reviewers raised other concerns in their reviews that they want addressed, such as discussing compatibility with recent ORAM models and clarifications on the implementation. Please refer to the weak points and detailed comments in the reviews.
    \item MRD3: \textit{Secure Protocol Compatibility and Implementation} 

    We added Section~\ref{sec:implementation} to show how \sysname is protocol agnostic and can support multiple secure computation protocols. We added an implementation using a state-of-the-art circuit model protocol, EMP~\cite{emp-toolkit}, and provide experimental results in Figures~\ref{fig:end-to-end-emp} and~\ref{fig:emp}. In the added text, we generalize our operator cost model to capture the performance behavior of both RAM model and circuit model protocols, as well as provide specific implementation details for how to integrate secure computation protocols with \sysname.  

\end{itemize}

\ \\
{\bf \large{Reviewer 2 Comments}}
\begin{itemize}
    %W1: The trust model is not adequately discussed, both at a high level, without a clear separation between what lies with the Honest Broker and what is assigned to the Data Owners, and at the low level, with a limited description of the roles of SMC and ORAM in the architecture.
    \item R2W1: \textit{Trust Model and Protocol Clarification}

    We added Sections~\ref{sec:privacygoals} and~\ref{sec:implementation} to clarify our trust model and better define the roles and implementation of the computation parties. We use secure computation protocols to ensure that the data views in Table 1 are satisfied. For more details, please see MRD1. 

    %W2: Limited consideration is offered about the impact of the destruction of the privacy budget as queries are executed over tables.
    \item R2W2: \textit{Privacy Budget Destruction}
    
    We added Section~\ref{sec:multiplequeries} to discuss the impact of privacy budget destruction as multiple queries are executed. The privacy loss of \sysname for answering multiple queries are analyzed using sequential composition (Theorem~\ref{theorem:seqcomp}) as it is general and easy to compute. There are two potential approaches for minimizing privacy loss: (i) applying advanced composition theorems that give tighter bounds on privacy loss under certain conditions~\cite{pdtextbook14} or (ii) optimizing privacy budget allocation across the operators of a set of predefined queries~\cite{McKenna:2018:OEH:3231751.3242939}. These two approaches are orthogonal to our work and it is non-trivial to extend them in the \mpc setting. We leave them for future work.
    
    %W3: The approach only considers the integration of data controlled by two authorities.
    \item R2W3: \textit{$M$-Party Support} 
    
    We added Section~\ref{sec:m-party} to examine how to extend \sysname from two parties to $M$ parties by leveraging the associativity of its operators. For more details, please see MRD2.
    
    %W4: The implementation does not use recent and more efficient ORAMs.
    \item R2W4: \textit{Secure Protocol Compatibility}
    
    We added Section~\ref{sec:implementation} to discuss how \sysname can support multiple secure computation protocols. We provide implementations of both RAM model and circuit model protocols, along with a discussion of the necessary operator cost model information. \sysname can support more recent ORAM implementations such as DORAM~\cite{Doerner2017} by summarizing their cost behavior as in Table~\ref{tbl:io-cost} and using those operator costs in our cost model. For more details, please see MRD3. 

\end{itemize}

\ \\
{\bf \large{Reviewer 4 Comments}}
\begin{itemize}
    %W1. D1. The description of the threat model is unclear. All parties and potential adversaries should be elaborated in more details, including their roles, abilities and goals. The privacy leakage model should also be presented. 
    \item R4W1,R4D1: \textit{Threat Model Clarification}
    
    We added Section~\ref{sec:privacygoals} to clarify our threat model and better define the roles of the computation parties. We use secure computation protocols to ensure that the data views in Table~\ref{table:trustmodel} are satisfied. For more details, please see MRD1.
    
    %W2. The novelty of the proposed new DDF is incremental. 
    \item R4W2: \textit{Novelty}
    
    We updated the introduction to better summarize our contributions. \sysname is the first system for private data sharing that combines differential privacy with \mpc for query performance optimization. We introduce: 1) a query processing engine that offers tunable, controlled information leakage to control the trade-off between privacy, accuracy, and performance, 2) a computational differential privacy mechanism that securely executes relational operators while minimizing \mpc overhead, 3) a novel algorithm that optimally allocates and applies differential privacy during query execution instead of only at the output, and 4) a protocol-agnostic cost model that approximates the large, and non-linear, computation overhead of \mpc. 
    
    %W3. The privacy sacrifice is not sufficiently evaluated. 
    %The experiments mainly measure the execution time performance. More results should be provided to explain how much privacy is sacrificed in order to achieve the desired speedup of query processing.
    \item R4W3,R4D5: \textit{Privacy Sacrifice Evaluation}
    
    We added Figures~\ref{fig:tradeoff} and~\ref{fig:accuracy} to discuss a wider range of privacy impacts on performance and accuracy. We also added Section~\ref{sec:multiplequeries} to discuss the impact of privacy budget destruction as multiple queries are executed. For more details, please see R2W2.
    
    %D2. There are contradictions in the paper. From Section 3 and Figure 2, there is no interaction between the honest broker and data owners or ORAM. However, in Section 5, while executing Algorithm 1, “\sysname looks at the intermediate result and calculates a new, differentially-private size for the ORAM” (function Resize), which means there are interactions between the honest broker and ORAM. Also, in the optimal budget splitting, intermediate results should be sent to \sysname which distributes the privacy budget for each operator.
    \item R4D2: \textit{Federation Role Clarification}

    In Section~\ref{sec:design}, we clarify the roles of the client, the coordinator and the data owners during query execution. Algorithm~\ref{algo:sw} shows how the data owners privately calculate the new differentially-private ORAM size with no assistance from the coordinator. In addition, intermediate results are created and accessed by the data owners alone. The only data sent to the coordinator are the final query results, which it decrypts upon receipt and then passes to the client.
    
    %D3. If there are interactions between \sysname and ORAM, extra costs are paid. Why not abandoning SMC/ORAM and using \sysname as a trusted third party directly? 
    \item R4D3: \textit{\sysname as Trusted Third Party}
    
    In Section~\ref{sec:privacygoals}, we discuss the trust model of private data federations, including how we do not use a trusted third party for execution. If we were to use \sysname as a trusted third party, the coordinator would learn the private data of the data owners, thereby violating the trust model described in Table~\ref{table:trustmodel}.
    
    %D4. In the experiments, only two private data owners are involved in the DDF. What about multiple data providers as in a typical DDF? 
    \item R4D4: \textit{$M$-Party Support}
    
    We added Section~\ref{sec:m-party} to examine how to extend \sysname from 2 parties to $M$ parties by leveraging the associativity of our operators. For details, please refer to MRD2 to see our discussion.
    
    \item R4D6: \textit{Small Errors}
    
    We corrected the errors in the text and thank the reviewer for bringing them to our attention.
\end{itemize}

\ \\
{\bf \large{Reviewer 5 Comments}}
\begin{itemize}
    %W1. Limited evaluation.
    %The first shortcoming is that evaluation is fairly simplistic. While it is true that real-world datasets and queries were used, it is also true that these queries were fairly simple and the datasets were tiny: a 15GB dataset is less than 25 percent of the main memory of one of the servers the authors used. I would welcome a study that scales the input size and queries -- even if the input size and queries are synthetically generated to provide more knobs in testing performance.
    \item R5W1: \textit{Limited Evaluation}
    
    We added Figure~\ref{fig:emp} to evaluate \sysname over larger datasets. We developed a synthetic data generator to scale up the input dataset sizes up to 50x the original data size of 15 GB, giving us an effective data size of 750 GB.  Regarding the query workloads, we use simpler, non-nested queries to better isolate the improvements due to \sysname in our experiments, shown in Figure~\ref{fig:join-scaling}. We also include an additional discussion in Sections~\ref{sec:join-scaling} and~\ref{sec:data-scaling} on how these experiments scale out with more complex workloads. 
    
    %W2. While the design section is detailed, there is little information provided for implementation. 
    %There is little information in terms of implementation. The authors only state they implemented this in a DBMS, but then stop at that. However, this is crucial for repeatability and to gauge the applicability of the approach. For instance, the system the authors used uses an exhaustive enumeration algorithm when exploring the search space of a query. Does the cost model reduce the need for such an approach? What changes were necessary in the storage engine/memory representation of the system to implement the proposed memory model? These are all important factors to present and consider when gauging the impact of the approach.
    \item R5W2: \textit{Federation Implementation}
    
    We have added algorithm details for \sysname in Section~\ref{sec:design}, as well as specific discussions of how we implement secure computation protocols using our cost model in Section~\ref{sec:implementation}. We discuss how \sysname is a flexible computation layer that supports a wide range of private data federations and database engines.  The only requirements are that the private data federation process queries as operator trees and that the underlying database engine supports SQL queries. 
    
    %W3. No validation of the proposed cost model.
    %The authors propose a cost model for their methodology, but they do not validate that cost model. I do appreciate the complexity and the fact that cost models do not necessarily need to be highly accurate, but rather aid the optimizer to make the correct decisions, but some notion of validation is necessary for the results of the cost model to be convincing.
    \item R5W3: \textit{Cost Model Evaluation}

    We have adjusted Figures~\ref{fig:speedup} and~\ref{fig:aspirin-operator} to show that privacy budget allocation based on our cost model provides near best-case runtimes. In Section~\ref{sec:budget-splitting}, we calculate the correlation coefficients between the true execution time and the estimated execution time using our cost model for both the RAM model (.931) and the circuit model (.998). 
    
\end{itemize}
We thank the reviewers again for their thoughtful feedback and their consideration of this revision. 

\newpage
\setcounter{page}{1}

